Learning Sparsely Used Overcomplete Dictionaries via Alternating Minimization

We consider the problem of sparse coding, where each sample consists of a sparse linear combination of a set of dictionary atoms, and the task is to learn both the dictionary elements and the mixing coefficients. Alternating minimization is a popular heuristic for sparse coding, where the dictionary and the coefficients are estimated in alternate steps, keeping the other fixed. Typically, the coefficients are estimated via $\ell_1$ minimization, keeping the dictionary fixed, and the dictionary is estimated through least squares, keeping the coefficients fixed. In this paper, we establish local linear convergence for this variant of alternating minimization and establish that the basin of attraction for the global optimum (corresponding to the true dictionary and the coefficients) is $\order{1/s^2}$, where $s$ is the sparsity level in each sample and the dictionary satisfies RIP. Combined with the recent results of approximate dictionary estimation, this yields provable guarantees for exact recovery of both the dictionary elements and the coefficients, when the dictionary elements are incoherent.

==> lemmas.tex <==
\newcommand{\Xoip}{\elt{\Xstar}{p}{i}}
\newcommand{\dip}{\delta^p_i}
\newcommand{\Mip}{M^p_i}
\newcommand{\diq}{\delta^q_i}
\newcommand{\Miq}{M^q_i}
\newcommand{\djp}{\delta^p_j}
\newcommand{\Mjp}{M^p_j}
\newcommand{\e}{{\bf e}}

\section{Main Technical Lemmas}
\label{sec:technical}

In this section, we state and prove the main technical lemmas used in
our results.
\alekhcomment{This subsection below looks redundant now, perhaps good
  to integrate into assumptions.}

\subsection{ Generative Model for $\Xstar$}\label{sec:genmodel}
Let each $\Xoip=\dip\Mip, \ \forall 1\leq p\leq n,\ \forall 1\leq
i\leq r$ where $\Mip$ are i.i.d. random variables.  That is, $\Mip
\stackrel{i.i.d.}{\sim} \mathcal{D}$ where $\expec{\Mip}=\mu$ and
$\expec{(\Mip)^2}=\sigma^2+\mu^2$.  We make the following assumptions
as well:
\begin{enumerate}
  \item	$\mu^2+\sigma^2 = 1$, and
  \item	$|\Mip|\leq M$ a.s.
\end{enumerate}

Also, let $\supp(\Xstar_i)=[\supp^1_i\ \supp^2_i\ \dots\ \supp^s_i]$ be
obtained by sampling uniformly {\em without replacement} from
$[r]$. Hence, $\dip=1$ if $p \in \supp(\Xstar_i)$ and $0$ otherwise.

%be i.i.d. random variables, such that,
%\begin{equation}
%  \label{eq:xoip}
%  \dip=\begin{cases} 1 & \text{ w.p. } \frac{s}{r}\\ 0 & \text{ w.p. } 1-\frac{s}{r}.\end{cases}
%\end{equation}
%Similarly,

\subsection{Proofs of Technical Lemmas}

\begin{lemma}\label{lem:expectedcovariance}
Let $\col{\Xstar}{i}$ be sampled from model as described in
Section~\ref{sec:genmodel}. Also, let $\mu^2+\sigma^2=1$. Then,
\begin{align*}
  \Sigma \defas \expec{\col{\Xstar}{i}
    \trans{\col{\Xstar}{i}}}=\left(\frac{s}{r} -
  \frac{s(s-1)\mu^2}{r(r-1)} \right) \eye +
  \frac{s(s-1)\mu^2}{r(r-1)}\ones \trans{\ones}.
\end{align*}
\end{lemma}
\bprf

Note that, $\dip, 1\leq p\leq r$ all have same distribution. Hence, by
symmetry and linearity of expectation,
$\expec{\dip}=\frac{1}{r}\expec{\sum_{q=1}^r
  \diq}=\frac{s}{r}$. Similarly,
$\expec{(\dip)^2}=\frac{1}{r}\expec{\sum_{q=1}^r
  (\diq)^2}=\frac{s}{r}$. Also, $\expec{(\sum_{q=1}^r
  (\diq))^2}=\expec{\sum_{p,q}\dip\diq}=r\expec{(\dip)^2}+(r^2-r)\expec{\dip\diq}$. Hence,
$\expec{\dip\diq}=\frac{s(s-1)}{r(r-1)}$.

Now, recall that $\Xoip=\dip\Mip$. Now,  we first consider diagonal
terms of $\Sigma$:

\begin{equation}
  \Sigma_p^p = \expec{(\Xoip)^2} = \expec{(\dip)^2}\expec{(\Mip)^2} =
  \frac{s}{r}(\mu^2+\sigma^2) = \frac{s}{r}.
  \label{eq:sigmaii}
\end{equation}
%
Similarly, using indepdence of $\Xoip$ and $\elt{\Xstar}{j}{p}$,
off-diagonal terms of $\Sigma$ are given by:
%
\begin{equation}
  \label{eq:sigmaij}
  \Sigma_p^q = \expec{\dip\diq}\expec{\Mip}\expec{\Miq} =
  \frac{s(s-1)}{r(r-1)}\mu^2.
\end{equation}
%
Lemma now follows by using \eqref{eq:sigmaii} and \eqref{eq:sigmaij}.
\eprf

In particular, two consequences of the lemma which will be
particularly useful are about the extreme singular values of
$\Sigma$. Recalling that $2s \leq r$ and $\mu^2 \leq 1$ by assumption,
we obtain

\begin{equation}
  \singmin(\Sigma) \geq \frac{s}{2r}, \quad \mbox{and} \quad
  \singmax(\Sigma) \leq \frac{2s^2}{r}.
  \label{eqn:extreme-cov-pop}
\end{equation}

%% \alekhcomment{This below might be redundant given bounds on the
%%   singular values of $\Sigma$.}

%% We will also need properties of the inverse covariance matrix which we
%% describe next.

%% \begin{lemma}\label{lem:invexpectedcovariance}
%% Let $\col{\Xstar}{i}$ be sampled from model as described in
%% Section~\ref{sec:genmodel}. Also, let $\mu^2+\sigma^2=1$. Then,
%% \begin{align*}
%%   \inv{\Sigma} &= \frac{r}{s\left(1-\frac{(s-1)\mu^2}{(r-1)}\right)}
%%   \eye -
%%   \frac{r(s-1)\mu^2}{s(r-1)\left(1-\frac{(s-1)\mu^2}{(r-1)}\right)
%%     \left(1+\left(s+\frac{1}{r-1}\right)\mu^2\right)} \ones
%%   \trans{\ones}.
%% \end{align*}
%% \end{lemma}
%% \bprf
%% Using Sherman-Morrison formula along with
%% Lemma~\ref{lem:expectedcovariance}, we get:

%% \begin{align}
%%   \inv{\Sigma} = \frac{r}{s\left(1-\frac{(s-1)\mu^2}{(r-1)}\right)}
%%   \eye - \frac{r^2}{s^2\left(1-\frac{(s-1)\mu^2}{(r-1)}\right)^2}\cdot
%%   \frac{s(s-1) \mu^2}{r(r-1)}\cdot
%%   \frac{\ones\trans{\ones}}
%%        {1+\frac{r}{s\left(1-\frac{(s-1)\mu^2}{(r-1)}\right)}\frac{s(s-1)
%%            \mu^2}{r(r-1)}(\trans{\ones}\ones)}.
%% \end{align}
%% %
%% Lemma follows by simplifying the above given expression.
%% \eprf


We first restate a theorem from \cite{Vershynin2010}, which we will
heavily use in the sequel.

\begin{theorem}[Restatement of Theorem 5.44 from \cite{Vershynin2010}]
\label{thm:rand-matrix-spectralnorm-vershynin}
Consider a $r \times n$ matrix ${W}$ where each column ${w_i}$ of
${W}$ is an independent random vector with covariance matrix
${\Sigma}$. Suppose further that $\twonorm{w_i} \leq
\sqrt{u}$ a.s. for all $i$. Then for any $t \geq 0$, the following inequality
holds with probability at least $1 - r \exp\left(-ct^2\right)$:
\begin{align*}
  \twonorm{\frac{1}{n} W W^T - \Sigma} \leq
  \max\left(\twonorm{\Sigma}^{1/2}\gamma,\gamma^2\right) \mbox{ where
  } \gamma = t \sqrt{\frac{u}{n}}.
\end{align*}
Here $c>0$ is an absolute numerical constant. In particular, this inequality yields:
\begin{align*}
  \twonorm{W} \leq \twonorm{\Sigma}^\frac{1}{2}
  \sqrt{n} + t \sqrt{u}.
\end{align*}
\end{theorem}

We need the following results on concentration of empirical covariance
matrices.

\begin{lemma}\label{lem:empiricalcovariance-concentration}
Let the conditions given in Lemma~\ref{lem:invexpectedcovariance}
hold.  There exists a universal constant $C$ such that w.p. $\geq
1-r\exp(-\frac{C \delta^2 n \spindex}{r M^2})$, we have:
\begin{align*}
  \twonorm{\frac{1}{n}\Xstar \trans{\Xstar} - \Sigma} \leq
  \max\left(\sqrt{2}\delta, \delta^2\right) \frac{s^2}{r}.
\end{align*}
In particular, w.p. $\geq 1-r\exp(-\frac{C n}{r M^2})$, we have the
bounds
\begin{align*}
   \twonorm{\Xstar}\leq 2\sqrt{\frac{ns^2}{r}} \quad \mbox{and} \quad
   \singmin(\Xstar) \geq \sqrt{\frac{n\spindex}{4r}}.
\end{align*}
\end{lemma}

\bprf

Note that, $\|\Xstar_i\|_2\leq \sqrt{s}M$. Also, $\|\Sigma\|_2\leq
\frac{s}{r}+\frac{s(s-1)\mu^2}{r-1}\leq \frac{2s^2}{r}$.  Using
Theorem~\ref{thm:rand-matrix-spectralnorm-vershynin} with $t =
\delta\sqrt{\frac{n\spindex}{rM^2}}$, we obtain:

$$\twonorm{\frac{1}{n}\Xstar \trans{\Xstar} - \Sigma} \leq
\max\left(\sqrt{2}\delta, \delta^2\right) \frac{s^2}{r},$$
%
w.p. greater than $1 - r \exp\left(-\frac{C \delta^2 n \spindex}{r
  M^2}\right)$. In order to obtain the second part, we apply the first
part of the lemma with $\delta = 1/4\sqrt{2}$ as well as
Lemma~\ref{lem:expectedcovariance} to bound the largest and smallest
singular values of $X\trans{X}/n$. Taking square roots completes the
proof.

\eprf

%% \alekhcomment{The lemma below seems redundant since we can use
%%   singular value bounds from above.}

%% \begin{lemma}\label{lem:invempiricalcovariance-concentration}
%% Let the conditions given in Lemma~\ref{lem:invexpectedcovariance}
%% hold. Also, let $r\geq 2 \spindex$. Then, the following holds w.p.
%% $\geq 1-r\exp\left(-\frac{C\delta^2n}{8srM^2}\right)$:
%% $$\twonorm{\inv{\left(\frac{1}{n}\Xstar \trans{\Xstar}\right)} - \inv{\Sigma}}
%% 	\leq \frac{2 r}{s}\cdot \frac{\delta}{1-\delta},\ \forall \delta\leq 1.$$
%% %% In particular, the following holds w.p. $\geq 1-r \exp(-10\log n)$,
%% %% \begin{align*}
%% %%   \twonorm{\inv{\left(\frac{1}{n}\Xstar \trans{\Xstar}\right)} - \inv{\Sigma}}
%% %% 	\leq  \frac{2r}{s}\cdot \sqrt{\frac{100s r\log n}{Cn}}M.
%% %% \end{align*}
%% %% Furthermore, assuming $n\geq C' s r^2 \log^2 r$, we get w.p. $\geq 1-r/n^{10}$:
%% %% \begin{align*}
%% %%   \twonorm{\inv{\left(\frac{1}{n}\Xstar \trans{\Xstar}\right)} - \inv{\Sigma}}
%% %% 	\leq  \frac{\sqrt{r}}{s}M.
%% %% \end{align*}
%% \end{lemma}

%% \bprf

%% Let $\frac{1}{n}\Xstar \trans{\Xstar}=\Sigma+E$. Note that using
%% Lemma~\ref{lem:empiricalcovariance-concentration}, $\twonorm{E}\leq
%% \max(\sqrt{2}\gamma, \gamma^2)\frac{s^2}{r}$ w.p. $\geq
%% 1-r\exp\left(-\frac{C \delta^2 n \spindex}{r M^2}\right)$. Selecting,
%% $\gamma=\frac{\delta}{2\sqrt{2}\cdot s}$ (where $\delta\leq 1$) we get
%% (w.p. $\geq
%% 1-r\exp\left(\frac{C\delta^2n}{8srM^2}\right)$): $$\twonorm{E}\leq
%% \frac{s}{2 r}\delta.$$ Also, using
%% Lemma~\ref{lem:invexpectedcovariance} and by using the assumption
%% $r\geq 2 \spindex$, we get: $\twonorm{\inv{\Sigma}}\leq \frac{2r}{s}$.
%% %$\|E\|_2\leq \sqrt{\frac{Cs^3\log n}{n\cdot r}}M$, w.p. $\geq

%% Let $\inv{\left(\frac{1}{n}\Xstar \trans{\Xstar}\right)}=\inv{\Sigma}-E_H$. That is, $E_H=\inv{\Sigma}(\eye-(\eye+\Sigma^{-1}E)^{-1})$. Now,
%% \begin{align}
%%   \|E_H\|_2\leq \|\inv{\Sigma}\|_2 \|\eye-(\eye+\Sigma^{-1}E)^{-1}\|_2 \stackrel{\zeta_1}{\leq} \frac{\|\inv{\Sigma}\|_2^2\|E\|_2}{1-\|\inv{\Sigma}\|_2\|E\|_2}\leq \frac{2r}{s}\cdot \frac{\delta}{1-\delta},\label{eq:covconc1}%\sqrt{\frac{Cs^3\log n}{n\cdot r}}M,
%% \end{align}
%% where $\zeta_1$ follows by using Sherman-Morrison-Woodbury identity and the last inequality follows by bound on $\|E\|_2$ and Lemma~\ref{lem:invexpectedcovariance}. Also, note that the above holds with w.p. $\geq 1-r\exp\left(\frac{C\delta^2n}{8srM^2}\right)$.
%% \eprf

Using the convergence of the covariance matrix of the sparsity
pattern, we obtain the following uniform convergence bound.

\begin{lemma}\label{lem:W-spectralnorm}
%Let $n\geq C s r^2 \log^2 r$. Then w.p. $\geq 1-1/n^{100}$,
For every $r \times n$ matrix $W$ s.t. $\supp(W)\subseteq
\supp(\Xstar)$, we have (w.p. $\geq 1-r\exp\left(-\frac{C
  n}{r}\right)$):
\begin{align*}
  \twonorm{W} \leq 2\|W\|_\infty\sqrt{\frac{s^2n}{r}}.
\end{align*}
\end{lemma}

\bprf
Since the support of $W$ is a subset of the support of $\Xstar$,
$W^p_i=\dip W^p_i$. Now,

\begin{align*}
\|W\|_2 &= \max_{u,v \|u\|_2=1, \norm{v}_2=1}\sum_{ip}W^p_iu^iv^p =
\max_{u,v \|u\|_2=1, \norm{v}_2=1}\sum_{ip}\dip W^p_iu^iv^p\\
&\leq \|W\|_\infty\cdot \max_{u,v \|u\|_2=1, \norm{v}_2=1}\cdot
\sum_{ip} \dip u^iv^p,
\end{align*}
%
where the inequality holds since the maximum inner product over the
all pairs $(u,v)$ from the unit sphere is larger than that over pairs
with $\row{u}{i}\row{v}{p} \geq 0$ for all $i,p$. Note that the last
expression is equal to $\norm{W}_\infty \trans{u}S(\Xstar)v$, where we
overload the notation $S(\Xstar)$ to also be the matrix with the
non-zero pattern of the matrix $\Xstar$. It suffices to control the
operator norm of this matrix for proving the lemma. This can indeed be
done by applying Lemmas~\ref{lem:expectedcovariance}
and~\ref{lem:empiricalcovariance-concentration} with $\mu = M = 1$ and
$\sigma = 0$. Doing so, yields with probability at least $\geq
1-r\exp\left(-\frac{C n}{r}\right)$

\begin{align*}
  \twonorm{W} \leq 2\|W\|_\infty\sqrt{\frac{s^2n}{r}},
\end{align*}
which completes the proof.
\eprf

In particular the following consequence of the above lemma would be
particularly useful in our proofs, where we apply the lemma to
matrices of the form $\delX = \Xnew - \Xstar$.

\begin{lemma}\label{lem:Xnew-spectralnorm}
For every $r \times n$ matrix $\Xnew$ s.t. $\supp(\Xnew)\subseteq
\supp(\Xstar)$, we have (w.p. $\geq 1-r\exp\left(-\frac{C n}{r}\right)
- r\exp\left(-\frac{C n}{rM^2}\right)$):
\begin{align*}
  \twonorm{\Xnew} \leq 2\cdot \left(1 + \infnorm{\Xnew -
    \Xstar}\right) \cdot \spindex \sqrt{\frac{n}{r}}.
\end{align*}
\end{lemma}

\bprf

Let $X=\Xstar+E_{\Xstar}$ where $\supp(E_{\Xstar})\subseteq
\supp(\Xstar)$. Hence, $\twonorm{\Xnew} \leq
\twonorm{\Xstar}+\twonorm{\Xnew-\Xstar}$.  Lemma follows directly
using Lemma~\ref{lem:empiricalcovariance-concentration} and
Lemma~\ref{lem:W-spectralnorm}.
\eprf

A useful version of the above lemma is when applied to matrices of the
form $\Xnew\trans{\Xnew}$. We will need control over the upper and
lower singular values of such matrices for our proofs, which we next
provide.

%The following lemma is a corollary of Lemma~\ref{lem:W-spectralnorm}.

\begin{lemma}\label{lem:Xnew-covariance-spectralnorm}
For every $r \times n$ matrix $\Xnew$ s.t. $\supp(\Xnew)\subseteq
\supp(\Xstar)$, we have w.p. $\geq 1-r\exp\left(-\frac{C n
}{r}\right)-r\exp\left(-\frac{C n }{rM^2}\right)$):

$$\twonorm{\Xnew\trans{\Xnew} - \Xstar\trans{\Xstar}}\leq
4\left(\infnorm{\Xnew - \Xstar} + \infnorm{\Xnew -
  \Xstar}^2\right)\cdot \frac{s^2n}{r}.$$

Further assuming $\norm{\Xnew - \Xstar}_\infty \leq 1/(64s)$, we have
with the same probability

\begin{equation*}
  \singmin(\Xnew \trans{\Xnew}) \geq \frac{ns}{8r}.
\end{equation*}
\end{lemma}

\bprf

Let $\Xnew=\Xstar+E_{\Xstar}$. Note that $\supp(E_{\Xstar})\subseteq
\supp(\Xstar)$. Now,

$$\|\Xnew\trans{\Xnew}-\Xstar\trans{\Xstar}\|_2 \leq
\|E_{\Xstar}\|_2(\|\trans{E_{\Xstar}}\|_2+2 \|\Xstar\|_2).$$ By
Lemma~\ref{lem:W-spectralnorm}, $\twonorm{E_{\Xstar}} \leq
2s\sqrt{\frac{n}{r}} \norm{\E_{\Xstar}}_\infty$ with probability at
least $\geq 1-r\exp\left(-\frac{C n}{r}\right)$. Combining this with
the bound on $\twonorm{\Xstar}$ from
Lemma~\ref{lem:empiricalcovariance-concentration} completes the
proof. The second statement now follows by combining the result with
our earlier lower bound on the minimum singular value of $\Xstar$ in
Lemma~\ref{lem:empiricalcovariance-concentration}.
\eprf

A particular consequence of this lemma which will be useful is a lower
bound on the diagonal entries of the matrix $X\trans{X}$. Indeed, we
see that under the assumption $\norm{\Xnew - \Xstar}_\infty \leq
1/(64s)$, with probability at least $1-r\exp\left(-\frac{C n
}{r}\right)-r\exp\left(-\frac{C n }{rM^2}\right)$ we have the lower
bound uniformly for all $p = 1,2,\ldots, r$

\begin{equation}
  \row{\Xnew}{p}\trans{\row{\Xnew}{p}} \geq \frac{ns}{8r}.
  \label{eqn:element-lb-xxtrans}
\end{equation}


We finally have the following concentration lemma.
\begin{lemma}\label{lem:dpchernoff}
Let $\dip$ be as defined in Section~\ref{sec:genmodel}. Then,
w.p. $\geq 1-\exp\left(-\frac{\delta^2}{3} ns^2/r^2\right)$:

\begin{enumerate}
  \item $\sum_{i=1}^n \dip \delta^q_i \leq (1+\delta) \frac{\spindex^2
    n}{r^2},\; \forall \; p\neq q$,
  \item $(1-\delta) \frac{\spindex n}{r}\leq \sum_{i=1}^n \dip \leq
    (1+\delta) \frac{\spindex n}{r},\; \forall \; p$,
  \item $(1-\delta) \frac{\spindex n}{r} \leq \sum_{i=1}^n \dip
    \left(\elt{M}{p}{i}\right)^2 \leq (1+\delta) \frac{\spindex
      n}{r},\; \forall \; p$, and
  \item $\sum_{i=1}^n \dip \abs{\elt{M}{p}{i}} \leq (1+\delta)
    \frac{\spindex n}{r},\; \forall \; p$.
\end{enumerate}
\end{lemma}

\bprf

Recall from the proof of Lemma~\ref{lem:expectedcovariance} that,
$\expec{\dip}=\frac{s}{r}$ and
$\expec{\dip\diq}=\frac{s(s-1)}{r(r-1)}, \forall p\neq q$. Also, these
random variables are independent for each $i$. Using Chernoff bound,
we get (w.p. $\geq 1-\exp(-\frac{\delta^2}{3}
ns^2/r^2)$): $$(1-\delta)n\frac{s}{r} \leq \sum_{i=1}^n \dip \leq
(1+\delta) n \frac{s}{r},\qquad \sum_{i=1}^n \dip \delta^q_i \leq
(1+\delta) n\frac{s^2}{r^2},\ \ \forall p\neq q.$$ The third part
follows similarly using Chernoff bound. The fourth part follows from
Chernoff bound as well after noting that

\begin{align*}
  \expec{\abs{\elt{M}{p}{i}}} \leq
  \left(\expec{\left(\elt{M}{p}{i}\right)^2}\right)^{\frac{1}{2}} \leq
  1,
\end{align*}
where the first step follows from Jensen's inequality.
\eprf

\begin{lemma}\label{lem:2-intersection}
For every $r\times n$ matrix $\Xnew$ s.t. $\supp(\Xnew)\subseteq
\supp(\Xstar)$, with probability at least \mbox{$1 -
  r\exp\left(-\frac{C n}{r}\right) - r\exp\left(-\frac{C
    n}{rM^2}\right) -\exp\left(-ns^2/(3r^2)\right)$} we have the
following bounds uniformly for all $p = 1,2,\ldots, r$
\begin{enumerate}
  \item $\twonorm{\elt{\left(\delX \trans{\Xnew}\right)}{\setminus
      p}{p}} \leq \left(1+\infnorm{\delX}\right)
    \frac{4\sqrt{2}\infnorm{\delX} s^2 n}{r^{\frac{3}{2}}}$, and
  \item $\twonorm{\row{\Xnew}{\setminus p}
    \trans{\left(\row{\Xnew}{p}\right)}} \leq
    \left(1+\infnorm{\delX}\right)^2\frac{4s^2n}{r^{\frac{3}{2}}}$,
\end{enumerate}
where $\delX \defas \Xnew - \Xstar$.
\end{lemma}

\bprf
Since $X$ has the same sparsity pattern as $\Xstar$, we can rewrite it
as $X^p_i=\dip X^p_i$. We start by proving the first part of the
lemma.

{\bf Proof of Part 1}: Wlog, we will prove the statement for $p = 1$.
Let $D$ denote the $n\times n$ diagonal matrix with
\begin{align*}
  \elt{D}{i}{i}=
	\left\{ \begin{array}{cc}
	1, &\mbox{if } \elt{\Xstar}{1}{i} \ne 0, \\
	0, &\mbox{otherwise.}
  \end{array}
\right.
\end{align*}
Using this notation, we have $\elt{\left(\delX
  \trans{\Xnew}\right)}{\setminus 1}{1} = \elt{\left(\delX D
  \trans{\Xnew}\right)}{\setminus 1}{1}$.  So, we have:

\begin{align*}
  \twonorm{\elt{\left(\delX \trans{\Xnew}\right)}{\setminus 1}{1}}
  &=   \twonorm{\elt{\left(\delX D
      \trans{\Xnew}\right)}{\setminus 1}{1}} \\
  &\leq \twonorm{\row{\left(\delX D\right)}{\setminus 1}}
  \twonorm{\col{\left(\trans{\Xnew}\right)}{1}} \\
  &\leq \twonorm{\row{\left(\delX D\right)}{\setminus 1}}
  \twonorm{\col{\left(\trans{\Xstar}\right)}{1} +
    \col{\left(\trans{\delX}\right)}{1}} \\
  &\stackrel{(\zeta_1)}{\leq} \twonorm{\row{\left(\delX
      D\right)}{\setminus 1}} \cdot \left(\sqrt{\frac{2sn}{r}} +
  \infnorm{\delX} \sqrt{\frac{2sn}{r}}\right),
\end{align*}
where $(\zeta_1)$ follows from Lemma~\ref{lem:dpchernoff}. In order to
control $\twonorm{\row{\left(\delX D\right)}{\setminus 1}}$, we
observe that it is a matrix with a random number of columns selected
by the matrix $D$. In particular, conditioned on $\set{i :
  \elt{D}{i}{i} = 1}$, the support of $\elt{\Xstar}{\setminus 1}{i}$
is independent over $s-1$ sparse vectors (and the support of $\delX$
is a subset of the support of $\Xstar$). Hence we can easily see that

\begin{align*}
  \P\left[ \twonorm{\row{\left(\delX D\right)}{\setminus 1}} > t
    \right] &\leq \P\left[ \twonorm{\row{\left(\delX
        D\right)}{\setminus 1}} > t \cap \frac{\spindex n}{2r} <
    \abs{\set{i : \elt{D}{i}{i} = 1}} < \frac{2\spindex n}{r} \right]\\
  &\qquad \qquad + \P\left[ \abs{\set{i : \elt{D}{i}{i} = 1}} \leq
    \frac{\spindex n}{2r} \cup  \abs{\set{i : \elt{D}{i}{i} = 1}} \geq
    \frac{2\spindex n}{r} \right].
\end{align*}
%
The first probability can be controlled by appealing to
Lemma~\ref{lem:W-spectralnorm}, while the second one is bounded
through Lemma~\ref{lem:dpchernoff} above. Doing so, we obtain with
probability at least \mbox{$1 - r\exp\left(-\frac{C n}{r}\right)
-\exp\left(-ns^2/(3r^2)\right)$}

\begin{align*}
  \twonorm{\row{\left(\delX D\right)}{\setminus 1}} \leq
  2\infnorm{\delX} \spindex \sqrt{\frac{\left(\frac{2\spindex
        n}{r}\right)}{r}}.
\end{align*}

This proves part 1.

{\bf Proof of Part 2}: The proof of this is similar to that of part
1. Wlog, assume $p=1$. We have:

\begin{align*}
  \twonorm{\row{\Xnew}{\setminus 1} \trans{\left(\row{\Xnew}{1}\right)}}
  &=  \twonorm{\row{\Xnew}{\setminus 1} D
    \trans{\left(\row{\Xnew}{1}\right)}} \\
  &\leq \twonorm{\row{\left(\Xnew D\right)}{\setminus 1}}
  \twonorm{\col{\left(\trans{\Xnew}\right)}{1}} \\
  &\stackrel{}{\leq} \twonorm{\row{\left(\Xnew D\right)}{\setminus 1}}
  \cdot 2\left(1+\infnorm{\delX}\right)\sqrt{\frac{sn}{r}}.
\end{align*}

For the first term above, we have:
\begin{align*}
  \twonorm{\row{\left(\Xnew D\right)}{\setminus 1}}
&\leq \twonorm{\row{\left(\Xstar D\right)}{\setminus 1}} +
  \twonorm{\row{\left(\delX D\right)}{\setminus 1}}
\end{align*}

The second term in this decomposition was controlled above and the
second one can be similarly bounded. Doing so, we obtain with
probability at least \mbox{$1 - r\exp\left(-\frac{C n}{r}\right) -
  r\exp\left(-\frac{C n}{rM^2}\right) -\exp\left(-ns^2/(3r^2)\right)$}

\begin{align*}
\twonorm{\row{\left(\Xnew D\right)}{\setminus 1}} \leq 2\spindex
\left(1+\infnorm{\delX}\right) \sqrt{\frac{2\spindex n}{r^3}},
\end{align*}
This proves the lemma.
\eprf

\begin{lemma}\label{lem:Schurcomplement}
  We have the following formula for matrix inversion:
\begin{align*}
  \inv{\left[ \begin{array}{cc} A & B \\
        C & D\end{array}\right]}
  = \left[ \begin{array}{cc}
      \inv{A} + \inv{A}BMC\inv{A} & - \inv{A}BM \\
      -MC\inv{A} & M \end{array} \right],
\end{align*}
where $M \defas \inv{\left(D - C \inv{A} B\right)}$ is the Schur
complement of $D$ in the above matrix.
\end{lemma}









% \subsection{Alternative Proof of Lemma~\ref{lem:bound-XXstarplus}}
% \bprf
% Let $V=\delX=X-\Xstar$. Then, using Sherman-Morrison-Woodbury identity:
% \begin{align}
%   \Xstar \pinv{\Xnew}&=\Xstar X^T\inv{(\Xstar\trans{\Xnew}+V\trans{\Xnew})}= \eye - V\inv{(I+\trans{\Xnew}\inv{(\Xstar\trans{\Xnew})}V)}\trans{\Xnew}\inv{(\Xstar\trans{\Xnew})}\nonumber\\
% &=\eye - V (\eye+E_1) \trans{\Xnew} (\frac{1}{n}\Sigma^{-1}+E_2),
% \end{align}
% where $E_1=\inv{(I+\trans{\Xnew}\inv{(\Xstar\trans{\Xnew})}V)}-\eye$ and $E_2=\inv{(\Xstar\trans{\Xstar}+\Xstar \trans{V})}-\frac{1}{n}\Sigma^{-1}$.
% Note that,
% \begin{align}&\|E_1\|_2\leq 2 \|X\|_2 \|\inv{(\Xstar\trans{X})}\|_2 \|V\|_2\leq 2\cdot 2CM s \sqrt{\frac{n}{r}} \cdot 64CM\frac{r}{n}M^4\cdot Cs \sqrt{\frac{n}{r}} \epsilon \leq 256C^2M^6s^2\epsilon.%,\nonumber\\
% %&\|E_2\|_2\leq \frac{2}{n^2}\|\Sigma^{-1}\|_2^2 \left(\|\Xstar\trans{\Xstar}-\frac{1}{n}\Sigma^{-1}\|_2+\|\Xstar\|_2\|\trans{V}\|_2\right)\leq \frac{2}{n^2}\cdot \frac{4r^2}{s^2}\cdot \left(4M^2 \sqrt{\frac{Cr^3\log r}{n^3 s^3}}+2C^2M\epsilon s^2\frac{n}{r}\right)
% \end{align}
% Now, consider $E_2$:
% \begin{align}
%   \|E_2\|_2=\|\frac{1}{n}\Sigma^{-1}\Xstar(\eye+\frac{1}{n}V^T\Sigma^{-1}\Xstar)^{-1}\frac{1}{n}V^T\Sigma^{-1}\|_2\leq \frac{2}{n^2} 2\epsilon nr \log^2 r.
% \end{align}
% \begin{align}
%   \|\Sigma^{-1}\Xstar\|_2\leq\|\frac{r}{s}\Xstar\|_2+\frac{2}{s}\sqrt{r}\|\Xstar^T\ones\|_2\leq \frac{r}{s}\sqrt{\frac{ns}{r}}+\frac{2\sqrt{r}}{s} s \log r \sqrt{n}\leq 2 \sqrt{nr}\log r.
% \end{align}

% Hence, $\forall p\neq q$:
% \begin{align}
%   |\e_q^T (\Xstar \pinv{\Xnew})\e_p|\leq |\frac{1}{n}\e_q^T V \trans{\Xnew} \Sigma^{-1}\e_p| +  |\e_q^T V \trans{\Xnew} E_2\e_p|+|\e_q^TV E_1 \trans{\Xnew} (\frac{1}{n}\Sigma^{-1})\e_p|+|\e_q^TV E_1 \trans{\Xnew}E_2\e_p|.
% \end{align}
% Now, we bound each of the four terms:
% \begin{align}
%   &\frac{1}{n}\e_q^T V \trans{\Xnew} \Sigma^{-1}\e_p\leq \frac{2r}{ns} |V^q \trans{(X^p)}| + \frac{2}{ns}|V^q \trans{\Xnew}\ones|\leq \epsilon M \frac{2r}{ns} \frac{2ns^2}{r^2}+\frac{2}{ns} \epsilon M C s \log r \frac{2n s}{r}\leq  \epsilon M \frac{4C s \log r}{r},\\
% &\e_q^T V \trans{\Xnew}E_2\e_p\leq \|V^qX\|_2\|E_2\|_2\leq \epsilon \sqrt{\frac{2ns^2}{r}}M,\\
% &|\e_q^TV E_1 \trans{\Xnew} (\frac{1}{n}\Sigma^{-1})\e_p|\leq \|V^q\|_2 \|E_1\|_2 \|\trans{\Xnew} (\frac{1}{n}\Sigma^{-1})\e_p\|_2\leq \epsilon \sqrt{\frac{2ns}{r}} \cdot 256C^2M^6s^2\epsilon\cdot \frac{1}{n} \frac{s}{r} M \sqrt{\frac{2ns}{r}}\leq \epsilon^2  \frac{256C^2M^6s^2 }{r^2},\\
% &|\e_q^TV E_1 \trans{\Xnew}E_2\e_p|\leq \|V^q\|_2 \|E_1\|_2 \|\trans{\Xnew}\|_2 \|E_2\|_2\leq \epsilon \sqrt{\frac{2ns}{r}}
% \end{align}
% \eprf
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "sparse-dict-altmin"
%%% End:


==> main-proof.tex <==
\section{Proof of Theorem~\ref{thm:main-altmin}}
\label{sec:proof-altmin}

In this section we will present the proof of
Theorem~\ref{thm:main-altmin}. The proofs of some auxilliary lemmas
and more technical arguments will be deferred to the appendices.

In order to keep the notation less cumbersome, we will track the
progress made in one iteration of Algorithm~\ref{algo:altmin}. For any
iteration $t$, we denote $\Aiter[t]$ as $\Aold$ and $\Aiter[t+1]$ as
$\Anew$. Similarly we denote $\Xiter[t]$ and $\Xiter[t+1]$ as $\Xold$
and $\Xnew$ respectively. Then the goal will be to show that $\Anew$
is closer to $\Astar$ than $\Aold$. For the purposes of our analysis,
we will find it more convenient to directly work with dot products
instead of $\ell_2$-distances (and hence avoid sign ambiguities). With
this motivation, we define the following notion of distance between
two vectors.

\begin{definition}\label{defn:dist-vector}
  For any two vectors $z,w \in \R^d$, we define the distance between
  them as follows:
\begin{align*}
  \distop{z}{w} \defas \sup_{v \perp w}
  \frac{\iprod{v}{z}}{\twonorm{v}\twonorm{z}} = \sup_{v \perp z}
  \frac{\iprod{v}{w}}{\twonorm{v}\twonorm{w}}.
\end{align*}
\end{definition}

This definition of distance suffices for our purposes due to the
following simple lemma

\begin{lemma}
  For any two unit vectors $u,v \in \R^d$, we have
  \begin{equation*}
    \min_{z \in \{-1,1\}} \norm{zu - v}_2 \leq \sqrt{2}\distop{u}{v}.
  \end{equation*}
  \label{lemma:ell2-to-distop}
\end{lemma}

\bprfof{Lemma~\ref{lemma:ell2-to-distop}}
The proof is rather straightforward. Suppose that $\iprod{u}{v}  > 0$
so that the minimum happens at $z = 1$. The other case is
identical. We can easily rewrite

\begin{align*}
  \norm{u - v}_2^2 = (2 - 2\iprod{u}{v}) \leq 2(1 - \iprod{u}{v}^2),
\end{align*}
%
where the final inequality follows since $0 \leq \iprod{u}{v} \leq
1$. Writing $u = \iprod{u}{v} v + v_{\perp}$, where
$\iprod{v_{\perp}}{v} = 0$, we see that

\begin{align*}
  1 = \norm{u}_2^2 = \iprod{u}{v}^2 + \norm{v_{\perp}}^2 =
  \iprod{u}{v}^2 + \distop{u}{v}^2.
\end{align*}
%
Substituting this into our earlier bound completes the proof.
\eprfof

The distance is naturally extended to matrices for our purposes by
applying it columnwise.

\begin{definition}\label{defn:dist-matrix}
  For any two $d\times r$ matrices $Z$ and $W$, we define the distance
  between them as follows:
\begin{align*}
  \distop{Z}{W} \defas \sup_{p \in [r]}
  \distop{\col{Z}{p}}{\col{W}{p}}.
\end{align*}
\end{definition}

Note that the normalization in the definition of $\distop{z}{w}$
ensures that we can apply the distance directly to the result of the
least-squares step without worrying about the effects of
normalization. This allows us to work with the closed-form expression
for $\Anew$

\begin{align}
  \Anew = \Ystar \pinv{\Xnew}
  &= \Astar \Xstar \pinv{\Xnew}. \label{eqn:update-A}
\end{align}

In order to establish Theorem~\ref{thm:main-altmin}, it suffices to
establish a recurrence relation of the form
\begin{align*}
  \distop{\Anew}{\Astar} < c \cdot \distop{\Aold}{\Astar},
\end{align*}
for some $c < 1$.
A natural strategy to show the above decay is as follows:
\begin{enumerate}
  \item	Using robustness properties of lasso, show:

    $$\twonorm{\Xnew - \Xstar} < c_{\textrm{lasso}} \cdot
    \left(\textrm{scaling factors}\right) \cdot \distop{\Aold}{\Astar}
    \mbox{ and,}$$
  \item Using results from matrix perturbation theory, show that

    $$\twonorm{\pinv{\Xnew}-\pinv{\Xstar}} < c_{\textrm{per}} \cdot
    \left(\textrm{scaling factors}\right) \cdot \twonorm{\Xnew -
      \Xstar},$$
\end{enumerate}
%
where $\left(\textrm{scaling factors}\right)$ are ones that depend on
the dimensions of the problem. It is tempting at this point to use the
definition of our updates~\eqref{eqn:update-A}, and obtain a
recurrence of the form
\begin{align*}
  \distop{\Anew}{\Astar} < c_{\textrm{lasso}} \cdot c_{\textrm{per}}
  \cdot \distop{\Aold}{\Astar},
\end{align*}
since $(\textrm{scaling factors})$ cancel each other. Used directly,
this approach does not quite yield the desired decay since the
resulting factors on the RHS are larger than 1. We now present a more
careful argument, replaces step 2 of the reasonining above with a more
careful analysis of the structure of our errors. In particular, we
will examine the deviations from identity of the matrix
$\Xstar\pinv{\Xnew}$. It will be shown that the off-diagonal entries
of this matrix are extremely small (the $\ell_2$-norm of a whole
column roughly scales as $1/\sqrt{r}$). On the other hand, the
diagonal entries can be much larger, but they only serve to rescale
the columns of $\Anew$ relative to those of $\Astar$. We now present a
couple of lemmas that formalize these steps, and then establish the
theorem using them. For ease of presentation, we will assume
throughout these arguments that the error bound
$\distop{\Aold}{\Astar} \leq \errt$ holds deterministically. The
necessary union bounds to ensure uniform probabiliies would be done in
the proof of the theorem.

Our first lemma characterizes the error in the update of $\Xnew$, as a
function of the error in our previous dictionary $\Aold$. For a
vector $v$ or a matrix $W$, we will use the shorthand $\nzset(v)$ and
$\nzset(W)$ to denote the set of non-zero entries of $v$ and $W$
respectively.

\begin{lemma}[Error in sparse recovery]
\label{lem:update-X}
  Let $\delX \defas \Xnew - \Xstar$. Assume that $2\mu_0s/\sqrt{d}
  \leq 0.1$ and $\sqrt{s\errt} \leq 0.1$ Then, we have:
\begin{enumerate}
  \item	$\nzset(\delX) \subseteq \nzset(\Xstar)$.
  \item $\infnorm{\delX} \leq 9s \cdot \distop{\Aold}{\Astar} \leq
    9s\errt$.
\end{enumerate}
\end{lemma}

\bprfof{Lemma~\ref{lem:update-X}}

In order to establish the lemma, we use a result of Candes regarding
the lasso estimator with deterministic noise. In particular, we use
the same argument as the proof of Proposition 3.3 in Agarwal et
al.~\cite{}, where it is shown that under the conditions of the lemma,
the matrix A satisfies the $2s$-RIP property with a constant at least
$0.1$. Further following their argument, we see that this guarantees
$\norm{\delX_i}_2 \leq 9s\errt$. Since this is also an infinity norm
error bound, we obtain the second part of the lemma. The proof of the
first part is further implied by the choice of our threshold at a
level of $9s\errt$, which ensures that any non-zero element in $\Xnew$
has $\abs{\elt{\Xstar}{i}{p}} \geq 0$ (since we would have
$\abs{\elt{\Xnew}{i}{p}} \leq 9s\errt$ by our inifinity norm bound
otherwise.  \eprfof

Using Lemma~\ref{lem:update-X} along with
Lemma~\ref{lem:W-spectralnorm} in Appendix~\ref{sec:technical} gives
us the following corollary, which finishes the first step in our proof
outline.
\begin{corollary}\label{cor:delX-spectralnorm}
With probability at least $1 - r\exp\left(-\frac{Cn}{r} \right)$, we
have the bound
\begin{align*}
  \twonorm{\delX} \leq 18 s^2 \sqrt{\frac{n}{r}}
  \distop{\Aold}{\Astar}.
\end{align*}
\end{corollary}
The next lemma, bounding the difference between $\pinv{\Xnew}$ and
$\pinv{\Xstar}$ finishes the second step of our outline.

%% \begin{lemma}[Perturbation of pseudo-inverses]
%% \label{lem:bound-perturbation-I}
%% Suppose the error at iteration $t$ satisfies $\errt \leq
%% 1/(288s^2)$. With probability at least $1 -
%% r\exp\left(-\frac{Cn}{rM^2} \right) - r\exp\left(-\frac{Cn}{r}
%% \right)$, we have the bound $\twonorm{\pinv{X}- \pinv{\Xstar}} \leq
%% \frac{415r}{n} \twonorm{\delX}.$
%% \end{lemma}


%% \bprfof{Lemma~\ref{lem:bound-perturbation-I}}
%% Using~\cite[Thm. 3.3]{stewart1977perturbation}, we have:
%% \begin{align*}
%% \twonorm{\pinv{\Xnew}- \pinv{\Xstar}} \leq 1.62 \max\{\twonorm{
%%   \pinv{\Xnew}}^2, \twonorm{\pinv{\Xstar}}^2 \}\twonorm{\delX}
%% \end{align*}
%% Note that $\twonorm{\delX}$ above is controlled by appealing to
%% Corollary~\ref{cor:delX-spectralnorm}. We now proceed to controlling
%% the other two terms.

%% \begin{align*}
%% \twonorm{ \pinv{\Xstar}} &= \twonorm{ \trans{\Xstar} \left( \Xstar
%%   \trans{\Xstar}\right)^{-1} }\\
%% &\leq \twonorm{ \Xstar} \twonorm{\left( \Xstar
%%   \trans{\Xstar}\right)^{-1} }.
%% \end{align*}

%% Both the terms in the above bound can be controlled by appealing to
%% Lemma~\ref{lem:empiricalcovariance-concentration}. The first term is
%% is directly bounded by the upper bound on $\singmax(\Xstar)$ in the
%% lemma, while the second one is bounded via the lower bound on
%% $\singmin(\Xstar)$. Doing so, we obtain with probability at least $1 -
%% r\exp\left(-\frac{Cn}{rM^2} \right)$

%% \begin{align}
%%   \twonorm{ \pinv{\Xstar}} \leq 2s \sqrt{\frac{n}{r}} \cdot
%%   \frac{4r}{ns}= 8\sqrt{\frac{r}{n}}
%%   \label{eqn:opnorm-pinv-xstar}
%% \end{align}
%% %
%% where $C$ is a universal constant that can change from line to line.

%% Next we bound $\twonorm{\pinv{\Xnew}}$. We first note using
%% Lemma~\ref{lem:empiricalcovariance-concentration} that $\Xstar$ is
%% full rank and $\sigma_{\textrm{min}}\left(\Xstar\right) >
%% \sqrt{\frac{sn}{4r}}$ with high probability.  Using
%% Corollary~\ref{cor:delX-spectralnorm}, since

%% $$\twonorm{\delX} < 18 s^2 \sqrt{\frac{n}{r}} \distop{\Aold}{\Astar} <
%% \frac{1}{16}\sqrt{\frac{n}{r}},$$
%% %
%% we see that $\textrm{rank}(\Xstar)=\textrm{rank}(\Xnew)$ with
%% probability at least $1 - r\exp\left(-\frac{Cn}{rM^2} \right) -
%% r\exp\left(-\frac{Cn}{r} \right)$. Using~\cite[Lemma 3.1]{Wedin73}, we
%% have:
%% \begin{align*}
%%   \twonorm{\pinv{\Xnew}} &\leq \frac{\twonorm{\pinv{\Xstar}}}{1-
%%     \twonorm{\pinv{\Xstar}} \twonorm{\delX}} \\
%%   &\leq \frac{8\sqrt{\frac{r}{n}}}{1 - 8\sqrt{\frac{r}{n}}
%%     \frac{1}{16}\sqrt{\frac{n}{r}}} \leq 16
%%   \sqrt{\frac{r}{n}}.
%% \end{align*}
%% This proves the lemma.
%% \eprfof

%% %% Plugging the results of Corollary~\ref{cor:delX-spectralnorm} and Lemma~\ref{lem:bound-perturbation-I} in
%% %% \eqref{eqn:update-A}, we obtain:
%% %% \begin{align*}
%% %%   \twonorm{\col{\Anew}{p}-\col{\Astar}{p}}
%% %% 	&= \twonorm{\Astar \Xstar \col{\left(\pinv{\Xnew}-\pinv{\Xstar}\right)}{p}} \\
%% %% 	&\leq \twonorm{\Astar} \twonorm{\Xstar} \twonorm{\pinv{\Xnew}-\pinv{\Xstar}} \\
%% %% 	&\leq \mu \sqrt{\frac{r}{d}} \cdot s\sqrt{\frac{n}{r}} \cdot 3.24 \sqrt{\frac{r}{n}}
%% %% 		\cdot c_{\textrm{lasso}} s \sqrt{\frac{n}{r}} \distop{\Aold}{\Astar} \\
%% %% 	&= 3.24 c_{\textrm{lasso}}\mu s^2 \sqrt{\frac{r}{d}} \distop{\Aold}{\Astar},
%% %% \end{align*}
%% %% which does not guarantee decay, since $3.24 c_{\textrm{lasso}}\mu s^2 \sqrt{\frac{r}{d}} > 1$ for the cases of our interest.
%% %% In order to over come this issue, we will do a much more careful analysis of the error terms and obtain the following
%% %% theorem.

Finished with the first two parts, we now move to the third part of
our proof approach, which considers the structure of the matrix
$\Xstar\pinv{X}$. Specifically, the next lemma will show how to control
the off-diagonal elements of this matrix carefully. We will be able to
use a much more obvious bound on the diagonal elements in proving the
theorem. For stating the lemma, we recall the notation
$\row{W}{\setminus p}$ which denotes all the elements of the matrix
$W$ except the $p_{th}$ row.

\begin{lemma}[Off-diagonal error bound]
  \label{lem:bound-XXstarplus}
Suppose $\infnorm{\delX} < \frac{1}{288 \spindex}$. Then with
probability at least \mbox{$1 - r\exp\left(-\frac{C n}{r}\right) -
  r\exp\left(-\frac{C n}{rM^2}\right)
  -\exp\left(-ns^2/(3r^2)\right)$}, we have uniformly for every $p \in
[r]$,
\begin{align*}
  \twonorm{\elt{\left(\delX \pinv{\Xnew}\right)}{\setminus p}{p}} =
  \twonorm{\elt{\left(\Xstar \pinv{\Xnew}\right)}{\setminus p}{p}}
  \leq \frac{1968 \spindex^2 \infnorm{\delX} }{\sqrt{r}}.
\end{align*}
\end{lemma}

\bprfof{Lemma~\ref{lem:bound-XXstarplus}}

For simplicity, we will prove the statement for $p=1$.
We first relate $\Xstar \pinv{\Xnew}$ to $\delX \pinv{\Xnew}$.

\begin{align*}
  \elt{\left(\Xstar \pinv{\Xnew}\right)}{\setminus 1}{1}
  &=   {\elt{\left(\left(\Xstar-\Xnew\right)
      \pinv{\Xnew}\right)}{\setminus 1}{1}} \\
  &=   -{\elt{\left(\delX \pinv{\Xnew}\right)}{\setminus 1}{1}} \\
  &=   -{\elt{\left(\delX \trans{\Xnew} \inv{\left(\Xnew
        \trans{\Xnew}\right)}\right)}{\setminus 1}{1}},
\end{align*}

where the first step follows from the fact that $\Xnew \pinv{\Xnew} =
\eye$.  This proves the first part of the lemma.  We now expand the
above as follows:

\begin{align*}
  \elt{\left(\delX \trans{\Xnew} \inv{\left(\Xnew
      \trans{\Xnew}\right)}\right)}{\setminus 1}{1}
  &= \elt{\left(\delX \trans{\Xnew}\right)}{\setminus 1}{1}
  \elt{\left(\inv{\left(\Xnew \trans{\Xnew}\right)}\right)}{1}{1}
  + \elt{\left(\delX \trans{\Xnew}\right)}{\setminus 1}{\setminus 1}
  \elt{\left(\inv{\left(\Xnew \trans{\Xnew}\right)}\right)}{\setminus
    1}{1}.
\end{align*}
Using triangle inequality, we have:
\begin{align}
  \twonorm{\elt{\left(\delX \trans{\Xnew} \inv{\left(\Xnew
        \trans{\Xnew}\right)}\right)}{\setminus 1}{1}}
  &\leq \underbrace{\abs{\elt{\left(\inv{\left(\Xnew
          \trans{\Xnew}\right)}\right)}{1}{1}}}_{\term_1}
  \underbrace{\twonorm{\elt{\left(\delX
        \trans{\Xnew}\right)}{\setminus 1}{1}}}_{\term_2} \nonumber \\
  &\qquad \qquad + \underbrace{\twonorm{\elt{\left(\delX
        \trans{\Xnew}\right)}{\setminus 1}{\setminus 1}}}_{\term_3}
  \underbrace{\twonorm{\elt{\left(\inv{\left(\Xnew
          \trans{\Xnew}\right)}\right)}{\setminus 1}{1}}}_{\term_4}.
  \label{eqn:bound-XXstarplus-triangle}
\end{align}

We now bound each of the above four quantities. We can easily bound
$\term_1$ via a spectral norm bound on
$\inv{(\Xnew\trans{\Xnew})}$. Doing so, we obtain with probability at
least $1-r\exp(-\frac{C \delta^2 n \spindex}{r M^2})$

\begin{align}
  \term_1 = \abs{\elt{\left(\inv{\left(\Xnew
        \trans{\Xnew}\right)}\right)}{1}{1}} \leq
  \twonorm{\inv{\left(\Xnew \trans{\Xnew}\right)}}
  &\stackrel{(\zeta_1)}{\leq} \frac{8r}{n \spindex},
	\label{eqn:bound-XXstarplus-I}
\end{align}

where $(\zeta_1)$ follows from
Lemma~\ref{lem:empiricalcovariance-concentration}. To bound $\term_2$,
we use Lemma~\ref{lem:2-intersection} and obtain with probability at
least \mbox{$1 - r\exp\left(-\frac{C n}{r}\right) -
  r\exp\left(-\frac{C n}{rM^2}\right) -\exp\left(-ns^2/(3r^2)\right)$}

\begin{align}
  \term_2 = \twonorm{\elt{\left(\delX \trans{\Xnew}\right)}{\setminus
      1}{1}} &\leq \frac{6 \infnorm{\delX} s^2 n
  }{r^{\frac{3}{2}}}, \label{eqn:bound-XXstarplus-II}
\end{align}
%
where we recall the assumption $\norm{\delX}_\infty \leq 1/(64s)$.
We now bound $\term_3$ as follows

\begin{align}
  \term_3 = \twonorm{\elt{\left(\delX \trans{\Xnew}\right)}{\setminus
      1}{\setminus 1}} \leq \twonorm{\elt{\left(\delX
      \right)}{\setminus 1}{\setminus 1}} \twonorm{\elt{\left(\Xnew
      \right)}{\setminus 1}{\setminus 1}} &\stackrel{(\zeta_1)}{\leq}
  2 \infnorm{\delX} \spindex \sqrt{\frac{n}{r}} \cdot 2 (1 +
  \infnorm{\delX} ) \spindex \sqrt{\frac{n}{r}}\nonumber \\
  &< \frac{ 6 \infnorm{\delX} \spindex^2 n
  }{r},\label{eqn:bound-XXstarplus-III}
\end{align}

where $(\zeta_1)$ follows from Lemmas~\ref{lem:W-spectralnorm} and
\ref{lem:Xnew-spectralnorm} (since $\nzset(\delX) \subseteq
\nzset(\Xnew) \cup \nzset(\Xstar) = \nzset(\Xstar)$). Finally, to
bound $\term_4$, we start by noting the following block decomposition
of the matrix $\Xnew\trans{\Xnew}$

\begin{equation*}
  X\trans{X} = \left[\begin{array}{cc} \row{X}{1}\trans{(\row{X}{1})}
      & \row{X}{1}\trans{(\row{X}{\setminus
          1})}\\ \row{X}{\setminus 1} \trans{\row{X}{1}} &
      \row{X}{\setminus 1}\trans{(\row{X}{\setminus 1})} \end{array}
    \right].
\end{equation*}
%
Given this block-structure, we can now invoke
Lemma~\ref{lem:Schurcomplement} (Schur complement lemma) to obtain

\begin{align*}
\elt{\left(\inv{\left(\Xnew \trans{\Xnew}\right)}\right)}{1}{\setminus
  1} =
-\frac{1}{\row{\Xnew}{1}\trans{\left(\row{\Xnew}{1}\right)}} B
\row{\Xnew}{\setminus 1}\trans{\left(\row{\Xnew}{1}\right)},
\end{align*}
%
where,

\begin{align}\label{eqn:Xinv-schur}
B \defas \elt{\left(\inv{\left(\Xnew
    \trans{\Xnew}\right)}\right)}{\setminus 1}{\setminus 1}%%  =
%% \inv{\left(\row{\Xnew}{\setminus 1}\trans{\left(\row{\Xnew}{\setminus
%%       1}\right)} -
%%   \frac{1}{\row{\Xnew}{1}\trans{\left(\row{\Xnew}{1}\right)}}
%%   \row{\Xnew}{\setminus 1}\trans{\left(\row{\Xnew}{1}\right)}
%%   \row{\Xnew}{1}\trans{\left(\row{\Xnew}{\setminus 1}\right)}
%%   \right)}
.
\end{align}
%
Using Lemma~\ref{lem:2-intersection} and
Equation~\ref{eqn:element-lb-xxtrans} we have with probability at
least\\ \mbox{$1 - r\exp\left(-\frac{C n}{r}\right) -
  r\exp\left(-\frac{C n}{rM^2}\right) -\exp\left(-ns^2/(3r^2)\right)$}

\begin{align}
  \twonorm{\elt{\left(\inv{\left(\Xnew
        \trans{\Xnew}\right)}\right)}{\setminus 1}{\setminus 1}} \leq
  \frac{1}{\abs{\row{\Xnew}{1}\trans{\left(\row{\Xnew}{1}\right)}}}
  \twonorm{B} \twonorm{\row{\Xnew}{\setminus
      1}\trans{\left(\row{\Xnew}{1}\right)}} \leq \frac{8r}{sn} \cdot
  \twonorm{B} \cdot \frac{5s^2 n}{r^{\frac{3}{2}}} =
  \frac{40s}{\sqrt{r}} \twonorm{M}.
  \label{eqn:bound-XXstarplus-IV-I}
\end{align}

Using the expression~\eqref{eqn:Xinv-schur} and the lower bound on
$\singmin(X)$ from Lemma~\ref{lem:Xnew-spectralnorm}, we also have the
following bound for $\twonorm{M}$ with probability at least \mbox{$1 -
  r\exp\left(-\frac{C n}{r}\right) - r\exp\left(-\frac{C
    n}{rM^2}\right)$}

\begin{align*}
  \twonorm{B} = \twonorm{\elt{\left(\inv{\left(\Xnew
        \trans{\Xnew}\right)}\right)}{\setminus 1}{\setminus 1}} &\leq
  \twonorm{\inv{\left(\Xnew \trans{\Xnew}\right)}} \leq \frac{8r}{n
    \spindex}.
\end{align*}
%
Plugging the above into \eqref{eqn:bound-XXstarplus-IV-I}, gives us:

\begin{align}
  \twonorm{\elt{\left(\inv{\left(\Xnew
        \trans{\Xnew}\right)}\right)}{\setminus 1}{\setminus 1}} &\leq
  \frac{40 \spindex}{\sqrt{r}} \cdot \frac{8r}{n \spindex} \leq
  \frac{320\sqrt{r}}{n}. \label{eqn:bound-XXstarplus-IV}
\end{align}

Combining \eqref{eqn:bound-XXstarplus-I},
\eqref{eqn:bound-XXstarplus-II}, \eqref{eqn:bound-XXstarplus-III} and
\eqref{eqn:bound-XXstarplus-IV}, we obtain with probability at least\\
\mbox{$1 - r\exp\left(-\frac{C n}{r}\right) - r\exp\left(-\frac{C
    n}{rM^2}\right) -\exp\left(-ns^2/(3r^2)\right)$}

\begin{align*}
  \twonorm{\elt{\left(\Xnew \pinv{\Xstar}\right)}{\setminus p}{p}} &\leq
  \frac{48 \infnorm{\delX}\spindex}{\sqrt{r}} + \frac{1920
    \infnorm{\delX}\spindex^2}{\sqrt{r}}\\
  &\leq \frac{1968 \spindex^2 \infnorm{\delX} }{\sqrt{r}}.
\end{align*}

\eprfof

Given these lemmas, We are now in a position to prove
Theorem~\ref{thm:main-altmin}




\bprfof{Theorem~\ref{thm:main-altmin}}

Let us recall the definition $\errt = \distop{\Aold}{\Astar}$. We will
show that for every $p \in [r]$, we have:
\begin{align}
  \distop{\col{\Anew}{p}}{\col{\Astar}{p}} \leq \frac{17712 \mu_1
    s^3}{\sqrt{d}} \errt.
  \label{eqn:distop-recur}
\end{align}
%
This suffices to prove the theorem by appealing to
Lemma~\ref{lemma:ell2-to-distop}.

Now fix any $w \perp \col{\Astar}{p}$ such that $\twonorm{w}=1$. We
first provide a bound on $\iprod{w}{\col{\Anew}{p}}$. We have with
high probability

\begin{align}
  \iprod{w}{\col{\Anew}{p}}
  = \trans{w} \Astar \Xstar \col{\pinv{\Xnew}}{p}
  &\stackrel{(\zeta_1)}{\leq} \twonorm{\trans{w} \Astar}
  \twonorm{\elt{\left(\Xstar\pinv{\Xnew}\right)}{\setminus p}{p}}
  \nonumber\\
  &\stackrel{(\zeta_2)}{\leq} \mu_1 \sqrt{\frac{r}{d}} \cdot \frac{1968
    \spindex^2 \infnorm{\delX}}{\sqrt{r}} \nonumber \\
  &= \frac{17712 \mu \spindex^3}{\sqrt{d}} \errt,
  \label{eqn:distop-upper}
\end{align}
%
where $(\zeta_1)$ follows from the fact that $\trans{w}
\col{\Astar}{p}=0$ and $(\zeta_2)$ follows from
Assumption~\ref{ass:spectral-bound} and
Lemma~\ref{lem:bound-XXstarplus}.

In order to bound $\distop{\Anew}{\Astar}$, it remains to show a lower
bound on $\norm{\Anew}_2$. This is again just algebraic given our
lemmas so far.

\begin{align*}
  \twonorm{\col{\Anew}{p}} = \twonorm{\Astar \Xstar \col{\pinv{\Xnew}}{p}}
  &= \twonorm{\Astar \left(\Xnew - \delX\right) \col{\pinv{\Xnew}}{p}} \\
  &\stackrel{(\zeta_1)}{=} \twonorm{\col{\Astar}{p} - \Astar \delX
    \col{\pinv{\Xnew}}{p}} \\
  &\geq \twonorm{\col{\Astar}{p}} - \twonorm{\Astar \col{\left(\delX
      \pinv{\Xnew}\right)}{p}},
\end{align*}
%
where $(\zeta_1)$ follows from the fact that $\Xnew \pinv{\Xnew} =
\eye$. We decompose the second term into diagonal and off-diagonal
terms of $\delX\pinv{\Xnew}$, followed by triangle inequality and
obtain

\begin{align*}
  \twonorm{\col{\Anew}{p}} &\geq 1 - \twonorm{\col{\Astar}{p}
    \elt{\left(\delX \pinv{\Xnew}\right)}{p}{p}
    + \col{\Astar}{\setminus p} \elt{\left(\delX
      \pinv{\Xnew}\right)}{\setminus p}{p}} \\
  &\geq 1 - \twonorm{\col{\Astar}{p}} \abs{\elt{\left(\delX
      \pinv{\Xnew}\right)}{p}{p}}
  - \twonorm{\col{\Astar}{\setminus p}} \twonorm{\elt{\left(\delX
      \pinv{\Xnew}\right)}{\setminus p}{p}} \\
  &\geq 1 - 1 \cdot \twonorm{\delX
    \trans{\Xnew}\inv{\left(\Xnew\trans{\Xnew}\right)}}
  - \twonorm{\col{\Astar}{\setminus p}} \twonorm{\elt{\left(\delX
      \pinv{\Xnew}\right)}{\setminus p}{p}} \\
  &\geq 1 - \underbrace{\twonorm{\delX} \twonorm{\trans{\Xnew}}
  \twonorm{\inv{\left(\Xnew\trans{\Xnew}\right)}} }_{\term_1}
  - \underbrace{\twonorm{\col{\Astar}{\setminus p}}
    \twonorm{\elt{\left(\delX \pinv{\Xnew}\right)}{\setminus
        p}{p}}}_{\term_2}
\end{align*}
%
It remains to control $\term_1$ and $\term_2$ at an appropriate
level. We start from $\term_1$. Note that $\twonorm{\delX}$ is bounded
by Corollary~\ref{cor:delX-spectralnorm}, while
$\twonorm{\trans{\Xnew}}$ is controlled by
Lemma~\ref{lem:Xnew-spectralnorm} (recall $\norm{\delX}_\infty \leq
1/(64s)$). Invoking Lemma~\ref{lem:Xnew-spectralnorm} to control
$\twonorm{\inv{X\trans{X}}}$, we obtain the following bound on
$\term_1$ with probability at least $1-r\exp\left(-\frac{C
  n}{r}\right) - r\exp\left(-\frac{C n}{rM^2}\right)$

\begin{equation*}
  \term_1 \leq 18 \errt \spindex^2 \sqrt{\frac{n}{r}} \cdot 3
  \spindex\sqrt{\frac{n}{r}} \cdot \frac{8r}{sn} = 432 \spindex^2
  \errt.
\end{equation*}
%
The second term $\term_2$ is directly controlled by
Lemma~\ref{lem:bound-XXstarplus}, yielding with probability at least\\
\mbox{$1 - r\exp\left(-\frac{C n}{r}\right) - r\exp\left(-\frac{C
    n}{rM^2}\right) -\exp\left(-ns^2/(3r^2)\right)$}
\begin{equation*}
  \term_2 \leq \mu_1 \sqrt{\frac{r}{d}} \frac{1968 \spindex^3
    \errt}{\sqrt{r}}
\end{equation*}
%
Putting all the terms together, we obtain that

\begin{align}
  \twonorm{\col{\Anew}{p}} \geq 1 - 9\spindex^2\left(48+\frac{1968
    \spindex \mu_1}{\sqrt{d}}\right)\errt \geq \frac{3}{4}.
  \label{eqn:distop-lower}
\end{align}
%
Combinig the bounds~\eqref{eqn:distop-upper}
and~\eqref{eqn:distop-lower} yields the desired
recursion~\eqref{eqn:distop-recur}. Appealing to
Lemma~\ref{lemma:ell2-to-distop} along with our setting of
$\errt$~\eqref{eqn:errt-seq} completes the proof of the
claim~\eqref{eqn:distop-recur}. Finally note that the error
probability in the theorem is obtained by using the fact that $M \geq
1$, and that the failure probability is purely incurred from the
structure of the non-zero entries of $\Xstar$, so that it is incurred
only once and not at each round. This avoids the need of a union bound
over all the rounds, yielding the result.
\eprfof



==> result.tex <==
\section{Algorithm and main result}
\label{sec:result}

In this section we will formally present our alternating minimization
method for dictionary learning, and present some recovery
guarantees. We start with the algorithm before presenting the precise
results.

\subsection{Alternating minmization for dictionary learning}
\label{sec:altmin-method}

At a high level, the method consists of alternating between a sparse
recovery step for estimating the coefficients given a dictionary, and
a least squares step for a dictionary given the coefficients. The
details of this approach are presented in
Algorithm~\ref{algo:altmin}. For ease of presentation in the
algorithm, we denote by $\thresh{\rho}{a}$ the thresholding operator

\begin{equation*}
  \thresh{\rho}{a} = \left\{ \begin{array}{cc} a & \mbox{if}~ \abs{a}
    > \rho\\
  0 & \mbox{otherwise}. \end{array} \right.
\end{equation*}
%
When the argument is a matrix or a vector, the thresholding is done
elementwise.

\begin{algorithm}[t]

  \caption{AltMinDict$(Y, \Aiter[0], \errt[0])$: Alternating minimization
    for dictionary learning}
  \label{algo:altmin}
  \begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{\textbf{Input: }}
    \renewcommand{\algorithmicensure}{\textbf{Output: }}
    \REQUIRE Samples $Y$, initial dictionary estimate $\Aiter[0]$, accuracy
    sequence $\errt$ and sparsity level $s$.
    \FOR{iterations $t = 0,1,2,\ldots, T-1$}
    \FOR{samples $i = 1,2,\ldots, n$}
    \STATE Estimate
    \begin{equation}
      \col{\Xiter[t+1]}{i} = \arg\min_{x \in \R^r} \norm{x}_1, \quad
      \mbox{subject to} \quad \norm{y_i - \Aiter x}_2 \leq
      \errt.
      \label{eqn:lasso}
    \end{equation}
    \ENDFOR
    \STATE Threshold: $\Xiter[t+1] = \thresh{9s\errt}{\Xiter[t+1]}$.
    \STATE Estimate $\Aiter[t+1] =
    Y\trans{\Xiter[t+1]}\inv{(\Xiter[t+1]\trans{\Xiter[t+1]})}$.
    \STATE Normalize: $\col{\Aiter[t+1]}{i} =
    \frac{\col{\Aiter[t+1]}{i}}{\norm{\col{\Aiter[t+1]}{i}}_2} $
    \ENDFOR
    \ENSURE $\Aiter[T]$
  \end{algorithmic}
\end{algorithm}

The sparse recovery step of Algorithm~\ref{algo:altmin} is based on
$\ell_1$-regularization, followed by thresholding. The thresholding
step is used to guarantee that the support set of our estimate
$\Xiter$ is a subset of the support set of the true coefficients
$\Xstar$ with high probability. The overall algorithmic scheme is
quite common to a variety of dictionary learning algorithms in the
prior work as well, and the exact lasso and least-squares steps can
also be replaced with other optimization methods for computational
reasons in practice (see e.g.~\cite{jenatton2010proximal}). As we will
discuss at the end, it might also be desirable to impose further
constraints on the structure of the non-zero entries in the matrix
$\Xiter$, although we leave such a development to future work.

\subsection{Linear convergence to the global optimum}
\label{sec:main-result}

We now present the main result of this section on the convergence
properties of Algorithm~\ref{algo:altmin}. For the purposes of the
result, we assume that Algorithm~\ref{algo:altmin} uses a sequence of
accuracy parameters such that $\errt[0] \geq \norm{\Aiter[0] -
  \Astar}_2$ and successively updates

\begin{equation}
  \errt[t+1] = \frac{25050 \mu_1 s^3}{\sqrt{d}} \errt.
  \label{eqn:errt-seq}
\end{equation}

We now state the main result.

\begin{theorem}\label{thm:main-altmin}
Suppose Assumptions~\ref{} hold, and assume that
Algorithm~\ref{algo:altmin} is initialized with the accuracy
sequence~\eqref{eqn:errt-seq}. Then with probability at least \mbox{$1
  - 2r\exp\left(-\frac{C n}{rM^2}\right)
  -\exp\left(-ns^2/(3r^2)\right)$}, the iterates $\Aiter$ satisfy for
uniformly all columns $i=1,2,\ldots, r$ and all $t = 1,2,\ldots, T$
\begin{align*}
  \min_{z \in \{-1,1\}} \norm{z\Aiteri    - \Astar_i}_2 \leq \errt.
  %% \distop{\Anew}{\Astar} \leq \frac{26912c_{\textrm{lasso}}\mu
  %%   s^2}{\sqrt{d}} \distop{\Aold}{\Astar}.
\end{align*}
\end{theorem}

The consequences of Theorem~\ref{thm:main-altmin} are powerful
combined with our Assumption~\ref{} and the
recurrence~\ref{eqn:errt-seq}. In particular, it is implied that with
high probability we obtain the recursion

\begin{equation*}
  \min_{z \in \{-1,1\}}\norm{z\col{\Aiter[t]}{i} -
    \col{\Astar}{i}}_2 \leq \norm{\Aiter[0] - \Astar}_2 2^{-t}.
\end{equation*}
%
The minimum over signs in the distance is taken since the algorithm
might return $-\col{\Astar}{i}$ instead of $\col{\Astar}{i}$ by
flipping the signs of the coefficients. Given the above bound, we need
at most $\order{ \log_2\frac{\epsilon}{\errt[0]}}$ in order to ensure
$\norm{z\col{\Aiter[T]}{i} - \col{\Astar}{i}}_2 \leq \epsilon$ for all
the dictionary elements $i = 1,2,\ldots, r$. Consequently, we get
exact recovery of the dictionary with finitely many samples. We
contrast this with the results of Arora et al.~\cite{}, who also
provide recovery guarantees to an arbitrary accuracy $\epsilon$, but
only if the number of samples is allowed to increase as $\epsilon$
decreases. Consequently, the result demonstrates a local linear
convergence of Algorithm~\ref{algo:altmin} to the globally optimal
solution despite the non-convexity in our formulation. Another way of
interpreting our result is that the global optimum has a \emph{basin
  of attraction} of size $\order{1/s}$ for our alternating
minimization procedure under these assumptions (since we require
$\errt[0] \leq 1/(64s)$).

